Improving GPU Performance Through Resource Sharing

Graphics Processing Units (GPUs) consisting of Streaming Multiprocessors (SMs) achieve high throughput by running a large number of threads and context switching among them to hide execution latencies. The number of thread blocks, and hence the number of threads that can be launched on an SM, depends on the resource usage--e.g. number of registers, amount of shared memory--of the thread blocks. Since the allocation of threads to an SM is at the thread block granularity, some of the resources may not be used up completely and hence will be wasted. We propose an approach that shares the resources of SM to utilize the wasted resources by launching more thread blocks. We show the effectiveness of our approach for two resources: register sharing, and scratchpad (shared memory) sharing. We further propose optimizations to hide long execution latencies, thus reducing the number of stall cycles. We implemented our approach in GPGPU-Sim simulator and experimentally validated it on several applications from 4 different benchmark suites: GPGPU-Sim, Rodinia, CUDA-SDK, and Parboil. We observed that with register sharing, applications show maximum improvement of 24%, and average improvement of 11%. With scratchpad sharing, we observed a maximum improvement of 30% and an average improvement of 12.5%.

==> Makefile <==
TGT=RegisterSharing

LATEX=pslatex
BIBTEX=bibtex
DVIPS=dvips
PS2PDF=ps2pdf -dEmbedAllFonts=true -dSubsetFonts=true -dEPSCrop=true -dPDFSETTINGS=/prepress 
LATEX_OPTS=-interaction=nonstopmode -halt-on-error
LATEX_OPTS=

NUM=""

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"


.PHONY: all clean


all: $(TGT).pdf

$(TGT).dvi : $(TGT).tex Sections/*.tex pstImages/*.tex RegSharing.bib
	$(LATEX) $(LATEX_OPTS) $(TGT).tex
	@if(grep "There were undefined references" $(TGT).log > /dev/null);\
	then \
		$(BIBTEX) $(TGT).aux; \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex; \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex; \
	fi
	@if(grep "Rerun" $(TGT).log > /dev/null);\
	then \
		$(LATEX) $(LATEX_OPTS) $(TGT).tex;\
	fi

$(TGT).pdf: $(TGT).ps
	$(PS2PDF) $(TGT).ps

$(TGT).ps: $(TGT).dvi
	$(DVIPS) -o $(TGT).ps $(TGT).dvi

.PHONY: clobber clean

clean:
	rm -rf $(TGT).aux $(TGT).log $(TGT).blg $(TGT).bbl $(TGT).dvi $(TGT).out

clobber: clean
	rm -rf $(TGT).pdf


